A high-resolution imaging of the collinear substructure of the proton

Accurate Standard Model predictions of proton-proton collisions are essential for interpreting the current and forthcoming experimental measurements from high-energy colliders. The quest for physics beyond the Standard Model is in fact strongly related to a reliable determination of systematic uncertainties, among which the theoretical ones have nowadays become a significant component. In particular, an important role is played by the universal Parton Distribution Functions (PDFs). This thesis presents a collection of studies aimed at improving the accuracy and precision of collinear PDF determinations. By employing the NNPDF methodology, we present recent polarized and unpolarized PDF fits including higher order QCD corrections and theoretical uncertainties. Additionally, we examine the presence of non-vanishing intrinsic charm and its phenomenological implications.

==> sections/icharm/subsec-3FNS_stability.tex <==
%---------------------------------------------------------------------
% From Nature SI
%---------------------------------------------------------------------

We now repeat the stability and uncertainty study of the previous section
\cref{sec:ic_stability_4FNS}, but for our final result, namely the intrinsic 
charm PDF. The main difference to be kept in mind is that the uncertainty now 
also includes the dominant MHOU, due to the matching condition required 
in order to determine the 3FNS PDF from the 4FNS result. 
In order to get a complete picture, we now add a further set of dataset variations.

\paragraph{Dependence on the input dataset.}
%
\cref{fig:charm_dataset_dep_nf3} displays the dataset variations shown in 
\cref{fig:charm_dataset_dep}, now for the intrinsic (3FNS) charm PDF, but 
with the total uncertainty now being the sum in quadrature of the PDF and 
MHO uncertainties, with the latter determined as the difference between
results obtained using NNLO and N$^3$LO matching.
%
Additionally, we also performed a few extra dataset variations: a fit without 
any $W, Z$ production data from ATLAS and CMS, a fit without jet data, a fit 
without $Z$ $p_T$ measurements, and a fit without HERA structure function data.
%
Note that the collider-only dataset includes both HERA electron-proton collider 
data and Tevatron and LHC hadron collider data, but not fixed-target DIS and DY 
production data.

Results are qualitatively very similar to those seen in the 4FNS, a consequence 
of the fact that we are focusing on the large-$x$ region where the effect of the 
matching is moderate, though now the presence of a valence-like peak in all 
determinations is even clearer, specifically for the DIS-only fit where it was 
less pronounced in the 4FNS.
%
As mentioned before, in the past, the main indication for intrinsic charm came from 
EMC data~\cite{Aubert:1982tt} on deep inelastic scattering with charm in the final 
state~\cite{Harris:1995jx}.
%
The results shown in \cref{fig:charm_dataset_dep_nf3}~(top right) indicate that 
the charm shape is now unchanged and EMC data contributes to a moderate reduction 
of uncertainties. 
%
Note however that the DIS-only determination exhibits larger uncertainties 
(up to factor 2) and point-by-point fluctuations, and is dominated by relatively 
old fixed-target measurements.
%
Comparison of all the dataset variations shows that, in terms of their impact 
on intrinsic charm, hadron collider data are generally more important that 
deep-inelastic data, that among the former the LHCb inclusive $W,Z$ data are 
playing a dominant role, and that jet observables also play a non-negligible role.

It should be stressed that the agreement between results found using DIS data 
and hadron collider data is highly nontrivial, since in the region relevant 
for intrinsic charm these determinations are based on disjoint datasets and 
are affected by very different theoretical and experimental uncertainties:
in particular, potential higher-twist effects in the DIS observables are highly 
suppressed for collider observables.
%
In this respect, a DIS-only determination of intrinsic charm is potentially affected 
by sources of theory uncertainties, such as higher twists, which are not accounted 
for in global PDF determinations.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!p]
    \centering
    \includegraphics[width=0.45\textwidth]{images/icharm/EMC_Quad_MHOU.pdf}
    \includegraphics[width=0.45\textwidth]{images/icharm/DIS_only_Quad_MHOU.pdf} \\
    \includegraphics[width=0.45\textwidth]{images/icharm/collider_only_Quad_MHOU.pdf}
    \includegraphics[width=0.45\textwidth]{images/icharm/noLHCb_Quad_MHOU.pdf} \\
    \includegraphics[width=0.45\textwidth]{images/icharm/noHERA_Quad_MHOU.pdf} 
    \includegraphics[width=0.45\textwidth]{images/icharm/noATLASCMSDY_Quad_MHOU.pdf} \\
    \includegraphics[width=0.45\textwidth]{images/icharm/nojets_Quad_MHOU.pdf}
    \includegraphics[width=0.45\textwidth]{images/icharm/noZpT_Quad_MHOU.pdf}
    \caption{
        Same as \cref{fig:charm_dataset_dep} for the intrinsic charm (3FNS) 
        PDF (top four plots), now also including four additional dataset variations: 
        no ATLAS and CMS $W, Z$ production data (third row left), no jet data 
        (third row right), no $Z$ $p_T$ measurements (bottom row left), no HERA 
        DIS data (bottom row right).
        %
        The error band indicates the PDF uncertainties combined in quadrature with the MHOUs.
    }
    \label{fig:charm_dataset_dep_nf3}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We conclude that the characteristic valence-like peak structure at large-$x$ predicted 
by non-perturbative intrinsic charm models (\cref{fig:charm_content_3FNS}) is always 
present even under very significant changes of the dataset.

% \paragraph{Dependence on the parametrization basis.}
% %
% \cref{fig:charm_basisdep_3FNS} displays the comparison between the intrinsic charm
% PDF determined with the default evolution basis choice, and the flavor basis. 
% Complete consistency of central values is found, with somewhat larger uncertainties 
% in the case of the flavor basis, due to the more challenging fitting environment in 
% this basis (see the discussion in~\cite{Ball:2021leu}).

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.49\textwidth]{images/icharm/Flavor_Basis_Quad_MHOU.pdf}
%     \caption{
%         Same as \cref{fig:charm_basisdep} for the intrinsic (3FNS) charm.
%     }
%     \label{fig:charm_basisdep_3FNS}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\paragraph{Dependence on the charm mass value.}
%
The study of the charm mass dependence is particularly interesting, because the 
intrinsic component should be independent of it, hence the residual dependence 
seen in \cref{fig:charm_fitted_mcdep} in the 4FNS, due to the mass dependence of 
the perturbative component that could not be reabsorbed in the fitting, should no 
longer be present. Results are shown in \cref{fig:mass_variations_Quad_MHOU}, and 
it is apparent that indeed the dependence on the charm mass has all but disappeared.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.49\textwidth]{images/icharm/mass_variations_Quad_MHOU.pdf}
    \includegraphics[width=0.49\textwidth]{images/icharm/mass_variations_ratio_Quad_MHOU.pdf}
    \caption{     
        Same as \cref{fig:charm_fitted_mcdep}, now for the intrinsic (3FNS) charm PDF. 
        Note that the intrinsic charm PDF is scale independent.
   }
   \label{fig:mass_variations_Quad_MHOU}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/icharm/subsec-ct14ic.tex <==
%---------------------------------------------------------------------
% From Nature SI
%---------------------------------------------------------------------

The possibility of an intrinsic charm component was recently studied in
~\cite{Hou:2017khm}, by modifying the CT14 PDF set, with the initial 4FNS 
charm PDF taken equal to the BHPS model~\cite{Brodsky:1980pb} form with 
the normalization fitted as a free parameter.
%
A 4FNS charm PDF with uncertainties at $Q=1.3$~GeV was then constructed by 
taking the BHPS model with best-fit normalization as central value (called 
the `BHPS1 model' in~\cite{Hou:2017khm}); the lower edge of the uncertainty 
band was taken to coincide with the standard CT14 charm PDF (i.e. the charm 
PDF determined by perturbative matching from the 3FNS to the 4FNS); the upper 
edge of the uncertainty band was taken as the BHPS model but with normalization 
fixed to the upper $90~\%$ CL limit (called the `BHPS2 model' in~\cite{Hou:2017khm}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.49\textwidth]{images/icharm/pdfplot-abs-lin-charm-q1p65gev.pdf}
    \includegraphics[width=0.49\textwidth]{images/icharm/pdfplot-abscharm-q1p65gev.pdf}
    \includegraphics[width=0.49\textwidth]{images/icharm/pdfplot-abscharm-q100gev.pdf}	
    \includegraphics[width=0.49\textwidth]{images/icharm/charm_momfrac_qdep_ct.pdf}
    \caption{
      The 4FNS charm PDF from~\cite{Hou:2017khm} compared to our result 
      (also in the 4FNS) at $Q=1.65$~GeV on a linear (top left) and logarithmic 
      (top right) scale in $x$, and at $Q=100$~GeV on a linear scale in 
      $x$ and as a ratio to our result (bottom left).
      %
      The momentum fraction corresponding to either case is also shown as 
      a function of $Q$ (bottom right). Note that for our result the uncertainty 
      band is the $68~\%$ CL PDF uncertainty, while for~\cite{Hou:2017khm} the 
      central curve (labeled CT14IC BHPS1) corresponds to the BHPS model 
      with best-fit normalization, the lower curve (labeled CT14) corresponds 
      to the default CT14 perturbative charm PDF and the upper curve 
      (labeled CT14IC BHPS2) corresponds to the BHPS model with normalization 
      at the upper $90~\%$ CL (see text). The value of the momentum fractions are 
      also provided in each case.
   }
   \label{fig:comparison_CT14}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The CT14IC charm PDF is compared to our result in \cref{fig:comparison_CT14}, 
at $Q=1.65$~GeV and $Q=100$~GeV, in the former case on both a logarithmic and linear 
scale in $x$ and in the latter case on a linear scale only, as a ratio to our default
result.
%
Note that the uncertainty band has a different interpretation in the two curves shown: 
for our result it is the $68\%$ CL PDF uncertainty, while for~\cite{Hou:2017khm} it corresponds 
to the model uncertainty estimated as described above.
%
In \cref{fig:comparison_CT14} we also quote the charm momentum fraction in each case, at 
the corresponding scale $Q$. As shown in \cref{fig:charm_content_3FNS} (right), our result for
the charm PDF is in good agreement with the BHPS model at large $x$. Correspondingly, for 
$x\gsim 0.3$ we find reasonably good agreement between our result and the central curve of
~\cite{Hou:2017khm}, which corresponds to a momentum fraction and thus a normalization of 
the charm PDF not too different from our result (see \cref{tab:momfrac_lowQ}).
%
Both the upper and lower curve from~\cite{Hou:2017khm} instead do not agree with our result 
within uncertainties: indeed the lower edge corresponds to the absence of intrinsic charm 
(which we exclude) and the upper edge to a momentum fraction which we exclude at more than 
the $5\sigma$ level (see \cref{tab:momfrac_lowQ}). 

For intermediate values $3\cdot10^{-3}\lsim x\lsim 0.3$ our result disagrees with that of 
~\cite{Hou:2017khm}, while at very small $x$ all results agree, the intrinsic charm being 
compatible with zero. The disagreement at intermediate $x$ is mostly due to the fact that 
in Ref.~\cite{Hou:2017khm} charm is assumed to take the BHPS form, which vanishes for $x\lsim 0.1$,
in the 4FNS at the low scale $Q=1.3$~GeV.
%
Due to perturbative evolution from $Q=1.3$~GeV to $Q=1.65$~GeV the charm PDF then develops 
the large bump that is seen in \cref{fig:comparison_CT14}, where we instead find that 
the 4FNS charm PDF is quite small.
%
This difference persists at large scales as seen in \cref{fig:charm_content_3FNS} (bottom left).

In terms of momentum fractions, shown in \cref{fig:charm_content_3FNS} (bottom right),
as already mentioned our result is compatible with the central value of~\cite{Hou:2017khm} 
within uncertainties; and also with the lower edge of ~\cite{Hou:2017khm} that corresponds 
to perturbative charm.
%
The upper edge of the prediction from~\cite{Hou:2017khm} is instead ruled out at more than 
$5\sigma$. 


==> tables/an3lo/tab-DY_datasets.tex <==
\begin{tabularx}{\textwidth}{Xccccc}
      \toprule
      Dataset
      & Ref.
      & $n_{\rm dat}$
      & Kin$_1$
      & Kin$_2$~[GeV]
      & $K$-factor N$^3$LO/NNLO
      \\
      \midrule
      ATLAS high-mass DY 7 TeV
      & \cite{Aad:2013iua}
      & 13
      & $|\eta_\ell|\leq 2.1$
      & $116\le m_{\ell\ell}\le 1500$
      & $d \sigma / d m_{\ell \ell}$
      \\
      ATLAS $Z$ 7 TeV ($\mathcal{L}=35$~pb$^{-1}$)
      & \cite{Aad:2011dm}
      & 8
      & $|\eta_\ell,y_Z|\leq 3.2$
      & $Q=m_Z$
      & $d \sigma / d m_{\ell \ell}~ (66 < m_{\ell \ell} < 150)$
      \\
      ATLAS $Z$ 7 TeV ($\mathcal{L}=4.6$~fb$^{-1}$) CC
      & \cite{Aaboud:2016btc}
      & 24
      & $|\eta_\ell,y_Z|\leq 2.5,3.6$
      & $Q=m_Z$ % $46 < m_{\ell \ell} < 116$
      & $d \sigma / d m_{\ell \ell}~(46 < m_{\ell \ell} < 116)$
      \\
      \midrule
      ATLAS $\sigma_{W,Z}^{\rm tot}$ 13 TeV
      & \cite{Aad:2016naf}
      & 3
      & ---
      & $Q=m_W,m_Z$
      & $\sigma$ \\
      \bottomrule
\end{tabularx}


==> tables/an3lo/tab_DIS_chi2.tex <==
\begin{tabularx}{\textwidth}{Xrccrccrcc}
  \toprule
  & \multicolumn{3}{c}{NLO}
  & \multicolumn{3}{c}{NNLO}
  & \multicolumn{3}{c}{aN$^3$LO} \\
  Dataset
  & $N_{\rm dat}$
  & no MHOU
  & MHOU
  & $N_{\rm dat}$
  & no MHOU
  & MHOU 
  & $N_{\rm dat}$
  & no MHOU
  & MHOU \\
  \midrule
  NMC $F_2^d/F_2^p$
  &  121 & 0.87 & 0.86
  &  121 & 0.87 & 0.88
  &  121 & 0.88 & 0.88 \\
  NMC $\sigma^{{\rm NC},p}$
  &  203 & 1.82 & 1.30
  &  204 & 1.57 & 1.33
  &  204 & 1.57 & 1.36 \\
  SLAC $F_2^p$
  &   33 & 1.64 & 0.74
  &   33 & 0.91 & 0.68
  &   33 & 0.93 & 0.72 \\
  SLAC $F_2^d$
  &   34 & 0.90 & 0.68
  &   34 & 0.61 & 0.54
  &   34 & 0.62 & 0.58 \\
  BCDMS $F_2^p$
  &  333 & 1.62 & 1.24
  &  333 & 1.40 & 1.29
  &  333 & 1.39 & 1.40 \\
  BCDMS $F_2^d$
  &  248 & 1.05 & 1.00
  &  248 & 1.01 & 0.99
  &  248 & 1.04 & 1.03 \\
  HERA I+II $\sigma_{\rm NC}\ e^-p$
  &  159 & 1.44 & 1.40
  &  159 & 1.40 & 1.39
  &  159 & 1.45 & 1.40 \\
  HERA I+II $\sigma_{\rm NC}\ e^+p$ ($E_p=460$~GeV)
  &  192 & 1.12 & 1.05
  &  204 & 1.09 & 1.04
  &  204 & 1.07 & 1.05 \\
  HERA I+II $\sigma_{\rm NC}\ e^+p$ ($E_p=575$~GeV)
  &  236 & 0.85 & 0.84
  &  254 & 0.93 & 0.88
  &  254 & 0.87 & 0.88 \\
  HERA I+II $\sigma_{\rm NC}\ e^+p$ ($E_p=820$~GeV)
  &   54 & 1.15 & 0.85
  &   70 & 1.12 & 0.95
  &   70 & 0.96 & 0.86 \\
  HERA I+II $\sigma_{\rm NC}\ e^+p$ ($E_p=920$~GeV)
  &  317 & 1.30 & 1.21
  &  377 & 1.31 & 1.25
  &  377 & 1.27 & 1.24 \\
  HERA I+II $\sigma_{\rm NC}^{c}$
  &   24 & 2.18 & 1.40
  &   37 & 1.96 & 1.75
  &   37 & 1.86 & 1.57 \\
  HERA I+II $\sigma_{\rm NC}^{b}$
  &   26 & 1.42 & 1.05
  &   26 & 1.44 & 1.11
  &   26 & 1.26 & 1.07 \\
  \midrule
  CHORUS $\sigma_{CC}^{\nu}$
  &  416 & 0.96 & 0.95 
  &  416 & 0.96 & 0.97
  &  416 & 0.97 & 0.98 \\
  CHORUS $\sigma_{CC}^{\bar{\nu}}$
  &  416 & 0.90 & 0.88
  &  416 & 0.88 & 0.87
  &  416 & 0.88 & 0.88 \\
  NuTeV $\sigma_{CC}^{\nu}$ (dimuon)
  &   39 & 0.24 & 0.22
  &   39 & 0.33 & 0.33
  &   39 & 1.27 & 1.28 \\
  NuTeV $\sigma_{CC}^{\bar{\nu}}$ (dimuon)
  &   36 & 0.43 & 0.35
  &   37 & 0.56 & 0.64
  &   37 & 0.63 & 0.59 \\
  HERA I+II $\sigma_{\rm CC}\ e^-p$
  &   42 & 1.34 & 1.19
  &   42 & 1.25 & 1.29
  &   42 & 1.29 & 1.34 \\
  HERA I+II $\sigma_{\rm CC}\ e^+p$
  &   39 & 1.26 & 1.22
  &   39 & 1.23 & 1.25
  &   39 & 1.27 & 1.28 \\
\bottomrule
\end{tabularx}


==> tables/an3lo/tab_DY_chi2.tex <==
\begin{tabularx}{\textwidth}{Xrccrccrcc}
  \toprule
  & \multicolumn{3}{c}{NLO}
  & \multicolumn{3}{c}{NNLO}
  & \multicolumn{3}{c}{aN$^3$LO} \\
  Dataset
  & $N_{\rm dat}$
  & no MHOU
  & MHOU
  & $N_{\rm dat}$
  & no MHOU
  & MHOU 
  & $N_{\rm dat}$
  & no MHOU
  & MHOU \\
  \midrule
  E866 $\sigma^d/2\sigma^p$ (NuSea)
  & 15 & 0.59 & 0.47
  & 15 & 0.52 & 0.51
  & 15 & 0.53 & 0.51 \\
  E866 $\sigma^p$ (NuSea)
  & 89 & 1.33 & 0.86
  & 89 & 1.59 & 1.00
  & 89 & 1.08 & 1.03 \\
  E605 $\sigma^d/2\sigma^p$ (NuSea)
  & 85 & 0.43 & 0.42
  & 85 & 0.46 & 0.45
  & 85 & 0.45 & 0.45 \\
  E906 $\sigma^d/2\sigma^p$ (SeaQuest)
  &  6 & 1.47 & 0.74
  &  6 & 0.97 & 0.90
  &  6 & 0.82 & 0.88 \\
  CDF $Z$ differential
  & 28 & 1.23 & 1.24
  & 28 & 1.23 & 1.18
  & 28 & 1.23 & 1.22 \\
  D0 $Z$ differential
  & 28 & 0.69 & 0.71
  & 28 & 0.64 & 0.64
  & 28 & 0.64 & 0.63 \\
  ATLAS low-mass DY 7 TeV
  &  4 & 0.69 & 0.66
  &  6 & 0.88 & 0.78
  &  6 & 0.78 & 0.76 \\
  ATLAS high-mass DY 7 TeV
  &  5 & 1.74 & 1.66
  &  5 & 1.60 & 1.67
  &  5 & 1.64 & 1.68 \\
  ATLAS $Z$ 7 TeV ($\mathcal{L}=35$~pb$^{-1}$)
  &  8 & 0.67 & 0.44
  &  8 & 0.58 & 0.57
  &  8 & 0.56 & 0.61 \\
  ATLAS $Z$ 7 TeV ($\mathcal{L}=4.6$~fb$^{-1}$) CC
  & 16 & 3.82 & 2.99
  & 24 & 1.80 & 1.68
  & 24 & 1.66 & 1.69 \\
  ATLAS $Z$ 7 TeV ($\mathcal{L}=4.6$~fb$^{-1}$) CF
  & 15 & 1.77 & 1.22
  & 15 & 1.07 & 1.02
  & 15 & 1.02 & 0.99 \\
  ATLAS low-mass DY 2D 8 TeV
  & 47 & 1.38 & 0.94
  & 60 & 1.23 & 1.08
  & 60 & 1.17 & 1.13 \\
  ATLAS high-mass DY 2D 8 TeV
  & 48 & 1.52 & 1.38
  & 48 & 1.11 & 1.08
  & 48 & 1.09 & 1.09 \\
  ATLAS $\sigma_{Z}^{\rm tot}$ 13 TeV
  & 1 & 0.12 & 0.41
  & 1 & 0.24 & 0.60
  & 1 & 0.24 & 0.66 \\
  ATLAS $Z$ $p_T$ 8 TeV ($p_T,m_{\ell\ell}$)
  & 41 & 1.08 & 0.91
  & 44 & 0.91 & 0.91
  & 44 & 0.89 & 0.89 \\
  ATLAS $Z$ $p_T$ 8 TeV ($p_T,y_Z$)
  & 28 & 0.87 & 0.52
  & 48 & 0.90 & 0.70
  & 48 & 0.77 & 0.68 \\
  CMS DY 2D 7 TeV
  &  88 & 1.29 & 1.11
  & 110 & 1.34 & 1.32
  & 110 & 1.34 & 1.36 \\
  CMS $Z$ $p_T$ 8 TeV
  &  28 & 1.66 & 1.47
  &  28 & 1.40 & 1.41
  &  28 & 1.35 & 1.39 \\
  LHCb $Z\to ee$ 7 TeV
  &   9 & 1.47 & 1.18
  &   9 & 1.65 & 1.53
  &   9 & 1.48 & 1.46 \\
  LHCb $Z \to \mu$ 7 TeV
  &  15 & 1.03 & 0.87
  &  15 & 0.80 & 0.73
  &  15 & 0.77 & 0.73 \\
  LHCb $Z\to ee$ 8 TeV
  &  17 & 1.58 & 1.38
  &  17 & 1.24 & 1.26
  &  17 & 1.31 & 1.27 \\
  LHCb $Z\to \mu$ 8 TeV
  &  15 & 1.25 & 1.06
  &  15 & 1.44 & 1.59
  &  15 & 1.60 & 1.60 \\
  LHCb $Z\to ee$ 13 TeV
  &  15 & 1.68 & 1.60
  &  15 & 1.72 & 1.80
  &  15 & 1.78 & 1.76 \\
  LHCb $Z\to \mu\mu$ 13 TeV
  &  16 & 1.10 & 1.11
  &  16 & 0.94 & 0.99
  &  16 & 0.99 & 0.94 \\
  \midrule
  D0 $W$ muon asymmetry
  &   8 & 2.42 & 2.17
  &   9 & 1.86 & 1.95
  &   9 & 2.07 & 2.03 \\
  ATLAS $W$ 7 TeV ($\mathcal{L}=35$~pb$^{-1}$)
  &  22 & 1.20 & 1.13
  &  22 & 1.11 & 1.12
  &  22 & 1.09 & 1.12 \\
  ATLAS $W$ 7 TeV ($\mathcal{L}=4.6$~fb$^{-1}$)
  &  22 & 2.18 & 2.13
  &  22 & 2.08 & 2.16
  &  22 & 2.16 & 2.10 \\
  ATLAS $\sigma_{W}^{\rm tot}$ 13 TeV
  &   2 & 0.16 & 0.54 
  &   2 & 1.21 & 1.60
  &   2 & 1.38 & 1.67 \\
  ATLAS $W^+$+jet 8 TeV
  &  15 & 0.26 & 0.28
  &  15 & 0.79 & 0.79
  &  15 & 0.73 & 0.73 \\
  ATLAS $W^-$+jet 8 TeV
  &  15 & 0.98 & 1.27
  &  15 & 1.49 & 1.45
  &  15 & 1.41 & 1.41 \\
  CMS $W$ electron asymmetry 7 TeV
  &  11 & 0.92 & 1.03
  &  11 & 0.84 & 0.85
  &  11 & 0.82 & 0.86 \\
  CMS $W$ muon asymmetry 7 TeV
  &  11 & 2.03 & 1.77
  &  11 & 1.71 & 1.73
  &  11 & 1.70 & 1.71 \\
  CMS $W$ rapidity 8 TeV
  &  22 & 0.93 & 0.74
  &  22 & 1.33 & 1.03
  &  22 & 1.11 & 1.08 \\
  LHCb $W \to \mu$ 7 TeV
  &  14 & 1.63 & 1.26 
  &  14 & 2.78 & 1.99
  &  14 & 2.12 & 2.03 \\
  LHCb $W \to \mu$ 8 TeV
  &  14 & 0.60 & 0.44
  &  14 & 0.97 & 0.92
  &  14 & 0.80 & 0.84 \\
\bottomrule
\end{tabularx}


==> tables/an3lo/tab_DY_chi2_kfactor.tex <==
\begin{tabularx}{\textwidth}{Xrccrcc}
  \toprule
  & \multicolumn{3}{c}{default}
  & \multicolumn{3}{c}{with N$^3$LO $K$-factors} \\
  Dataset
  & $N_{\rm dat}$
  & no MHOU
  & MHOU 
  & $N_{\rm dat}$
  & no MHOU
  & MHOU \\
  \midrule
  ATLAS high-mass DY 7 TeV
  &  5 & 1.64 & 1.68
  &  5 & 1.63 & 1.56 \\
  ATLAS $Z$ 7 TeV ($\mathcal{L}=35$~pb$^{-1}$)
  &  8 & 0.56 & 0.61 
  &  8 & 0.47 & 0.52 \\
  ATLAS $Z$ 7 TeV ($\mathcal{L}=4.6$~fb$^{-1}$) CC
  & 24 & 1.66 & 1.69 
  & 24 & 1.90 & 1.59 \\
  ATLAS $\sigma_{Z}^{\rm tot}$ 13 TeV
  & 1 & 0.24 & 0.66
  & 1 & 0.06 & 0.00 \\
  ATLAS $\sigma_{W}^{\rm tot}$ 13 TeV
  &   2 & 1.38 & 1.67 
  &   2 & 1.33 & 1.59 \\
\bottomrule
\end{tabularx}


==> tables/an3lo/tab_OTHER_chi2.tex <==
\begin{tabularx}{\textwidth}{Xrccrccrcc}
  \toprule
  & \multicolumn{3}{c}{NLO}
  & \multicolumn{3}{c}{NNLO}
  & \multicolumn{3}{c}{aN$^3$LO} \\
  Dataset
  & $N_{\rm dat}$
  & no MHOU
  & MHOU
  & $N_{\rm dat}$
  & no MHOU
  & MHOU 
  & $N_{\rm dat}$
  & no MHOU
  & MHOU \\
  \midrule
  ATLAS $\sigma_{tt}^{\rm tot}$ 7 TeV
  & 1 & 10.4 & 0.96
  & 1 & 4.50 & 2.40 
  & 1 & 2.78 & 2.05 \\
  ATLAS $\sigma_{tt}^{\rm tot}$ 8 TeV
  & 1 & 1.74 & 0.59
  & 1 & 0.02 & 0.03
  & 1 & 0.04 & 0.08 \\
  ATLAS $\sigma_{tt}^{\rm tot}$ 13 TeV ($\mathcal{L}$=139~fb$^{-1}$)
  & 1 & 3.82 & 0.96
  & 1 & 0.49 & 0.41
  & 1 & 0.51 & 0.44 \\
  ATLAS $t\bar{t}~\ell$+jets 8 TeV ($1/\sigma d\sigma/dy_t$)
  & 4 & 4.16 & 1.79
  & 4 & 3.13 & 3.70
  & 4 & 2.98 & 3.64 \\
  ATLAS $t\bar{t}~\ell$+jets 8 TeV ($1/\sigma d\sigma/dy_{t\bar t}$)
  & 4 & 8.93 & 3.73
  & 4 & 4.50 & 5.80
  & 4 & 4.26 & 4.92 \\
  ATLAS $t\bar{t}~2\ell$ 8 TeV ($1/\sigma d\sigma/dy_{t\bar t}$)
  & 4 & 1.94 & 1.76
  & 4 & 1.60 & 1.86
  & 4 & 1.66 & 1.80 \\
  CMS $\sigma_{tt}^{\rm tot}$ 5 TeV
  & 1 & 0.61 & 0.73
  & 1 & 0.02 & 0.01
  & 1 & 0.03 & 0.02 \\
  CMS $\sigma_{tt}^{\rm tot}$ 7 TeV
  & 1 & 5.27 & 1.30
  & 1 & 1.01 & 0.50
  & 1 & 0.60 & 0.34 \\
  CMS $\sigma_{tt}^{\rm tot}$ 8 TeV
  & 1 & 3.50 & 0.85
  & 1 & 0.26 & 0.17
  & 1 & 0.21 & 0.10 \\
  CMS $\sigma_{tt}^{\rm tot}$ 13 TeV
  & 1 & 0.75 & 0.26
  & 1 & 0.06 & 0.01
  & 1 & 0.04 & 0.05 \\
  CMS $t\bar{t}~\ell$+jets 8 TeV ($1/\sigma d\sigma/dy_{t\bar t}$)
  & 9 & 1.87 & 1.59
  & 9 & 1.21 & 1.59
  & 9 & 1.31 & 1.52 \\
  CMS $t\bar{t}$ 2D $2\ell$ 8 TeV ($1/\sigma d\sigma/dy_tdm_{t\bar t}$)
  & 15 & 2.03 & 1.89
  & 15 & 1.30 & 1.25
  & 15 & 1.28 & 1.37 \\
  CMS $t\bar{t}~2\ell$ 13 TeV ($d\sigma/dy_t$)
  & 10 & 0.78 & 0.69
  & 10 & 0.51 & 0.59
  & 10 & 0.55 & 0.60 \\
  CMS $t\bar{t}~\ell$+jet 13 TeV ($d\sigma/dy_t$)
  & 11 & 0.66 & 0.25
  & 11 & 0.60 & 0.66
  & 11 & 0.52 & 0.71 \\ 
  \midrule
  ATLAS incl. jets 8~TeV, $R=0.6$
  & 171 & 0.67 & 0.74
  & 171 & 0.68 & 0.64
  & 171 & 0.68 & 0.64 \\
  CMS incl. jets 8 TeV
  & 185 & 0.95 & 0.83
  & 185 & 1.19 & 0.95
  & 185 & 0.97 & 0.99 \\
  \midrule
  ATLAS dijet 7 TeV, $R=0.6$
  & 90 & 1.47 & 1.72
  & 90 & 2.14 & 1.69
  & 90 & 1.76 & 1.63 \\
  CMS dijet 7 TeV
  & 54 & 1.57 & 2.01
  & 54 & 1.79 & 1.74
  & 54 & 1.84 & 1.78 \\
  \midrule
  ATLAS isolated $\gamma$ prod. 13 TeV
  & 53 & 0.57 & 0.47
  & 53 & 0.76 & 0.67
  & 53 & 0.72 & 0.68 \\
  \midrule
  ATLAS single~$t$ $R_{t}$ 7 TeV
  & 1 & 0.43 & 0.29
  & 1 & 0.50 & 0.57
  & 1 & 0.51 & 0.58 \\
  ATLAS single~$t$ $R_{t}$ 13 TeV
  & 1 & 0.04 & 0.03
  & 1 & 0.06 & 0.07
  & 1 & 0.06 & 0.07 \\
  ATLAS single~$t$ 7 TeV ($1/\sigma d\sigma/dy_t$)
  & 3 & 0.83 & 0.84
  & 3 & 0.96 & 0.94
  & 3 & 0.97 & 0.97 \\
  ATLAS single~$t$ 7 TeV ($1/\sigma d\sigma/dy_{\bar t}$)
  & 3 & 0.06 & 0.06
  & 3 & 0.06 & 0.06
  & 3 & 0.06 & 0.06 \\
  ATLAS single~$t$ 8 TeV ($1/\sigma d\sigma/dy_t$)
  & 3 & 0.38 & 0.31
  & 3 & 0.25 & 0.26
  & 3 & 0.22 & 0.24 \\
  ATLAS single~$t$ 8 TeV ($1/\sigma d\sigma/dy_{\bar t}$)
  & 3 & 0.19 & 0.21
  & 3 & 0.19 & 0.19
  & 3 & 0.20 & 0.20 \\
  CMS single~$t$ $\sigma_{t}+\sigma_{\bar{t}}$ 7 TeV
  & 1 & 0.89 & 0.88
  & 1 & 0.74 & 0.84
  & 1 & 0.39 & 0.43 \\
  CMS single~$t$ $R_{t}$ 8 TeV
  & 1 & 0.15 & 0.08
  & 1 & 0.18 & 0.20
  & 1 & 0.18 & 0.21 \\
  CMS single~$t$ $R_{t}$ 13 TeV
  & 1 & 0.33 & 0.27
  & 1 & 0.36 & 0.38
  & 1 & 0.36 & 0.38 \\
\bottomrule
\end{tabularx}


==> tables/intro/CC_to_NC_dis_mapping.tex <==
\begin{tabularx}{0.7\textwidth}{c|c|c|c|c}
     & Parity & Channel & $C^{+}$ & $C^{-}$ \\
    \toprule
    \multirow{3}{*}{$F_2$, \ $F_L$, \ $2xg_1$} & \multirow{3}{*}{conserving} & $ns$ & $=$ NC & $\neq$ \\
                                &                  & $g$, $ps$ &  $=$ NC  & $\times$ \\
                                &                  & $pv$ &  $\times$  & $\times$ \\
    \midrule
    \multirow{3}{*}{$xF_3$, \ $g_L$, \ $g_4$}  & \multirow{3}{*}{violating} & $ns$ &  $=$ NC & $\neq$ \\
                                &                  & $g$, $ps$ &  $\times$  & $\times$ \\
                                &                  & $pv$ &  $=$ NC & $\times$ \\
    \bottomrule                                         
\end{tabularx}

==> tables/intro/dis_mellin_mapping.tex <==
\begin{tabularx}{0.45\textwidth}{c|c|c}
                               & NC, CC $+$ & CC $-$ \\
    \toprule
    $F_2$, \ $F_L$, \ $g_4$, \ $g_L$ & even-N & odd-N \\
    \midrule
    $xF_3$, \ $2xg_1$ & odd-N  & even-N \\
    \bottomrule                                         
\end{tabularx}
